Pooling And Attention: What Are Effective Designs For LLM-Based Embedding Models?

The significant advancements of Large Language Models (LLMs) in generative tasks have led to a growing body of work exploring LLM-based embedding models. While these models, employing different pooling and attention strategies, have achieved state-of-the-art performance on public embedding benchmarks, questions still arise about what constitutes an effective design for LLM-based embedding models. However, these models are often trained on different datasets, using different LLM base models or training settings. Moreover, evaluations on public embedding benchmarks often fail to report statistical significance, making it difficult to determine which designs truly contribute to final performance. This complicates the process for practitioners seeking optimal training recipes for LLM-based embedding models. In this study, we conduct a large-scale experiment by training a series of LLM-based embedding models using the same training data and base model but differing in their pooling and attention strategies. The results show that there is no one-size-fits-all solution: while bidirectional attention and an additional trainable pooling layer outperform in text similarity and information retrieval tasks, they do not significantly surpass simpler designs like EOS-last token pooling and default causal attention in clustering and classification tasks. Furthermore, we propose a new pooling strategy, Multi-Layers Trainable Pooling, which transforms the outputs of all hidden layers, rather than just the last layer, using a cross-attention network. This method proves to be statistically superior in text similarity and retrieval tasks compared to existing pooling methods. Overall, this paper sheds light on effective training strategies for LLM-based embedding models.

==> sections/main_tables/mteb.tex <==

\begin{table*}[ht]
\footnotesize
\centering
\begin{tabular}{@{}>{\raggedright\arraybackslash}m{5.5cm}cccccccc@{}}
\toprule
Model & STS & Clas. & Retr. & Clus. & Rera. & P. Cls. & Summ. & Avg.\\ \midrule
Casual-Mistral-7B\\ \quad + EOS Token Pooling & 0.8302 & \textbf{0.7244} & 0.5394 & \textbf{0.4503} & 0.5737 & 0.8605 & \textbf{0.3240} & 0.6146\\
Casual-Mistral-7B\\ \quad + \newmethod (EOS Token) & 0.8420 & 0.7211 & 0.5529 & 0.4486 & 0.5787& 0.8627 & 0.2996 & \textbf{0.6151}\\
Casual-Mistral-7B\\ \quad + \newmethod (Last Token) & 0.8406 & 0.7236 &0.5512 & 0.4283 & 0.5831& 0.8464 & 0.3115 & 0.6121\\
Casual-Mistral-7B\\ \quad + \newmethod (EOS Token) \\ \qquad - Layer Weights & 0.8431  & 0.7209 & 0.5496 & 0.4427 & 0.5720 & 0.8639 & 0.3097 & 0.6146\\ \hline
Bi-directional-Mistral-7B\\ \quad + \newmethod & \textbf{0.8468} & 0.7101 & \textbf{0.5620} & 0.4257 & 0.5812 & \textbf{0.8746} & 0.2946 & 0.6136\\
Bi-directional-Mistral-7B\\ \quad + \newmethod \\ \qquad - Layer Weights & +0.0166 & -0.0143 & +0.0226 & -0.0246 & +0.0075 & +0.0141 & -0.0294 & -0.001\\ \bottomrule
\end{tabular}
\caption{The benchmark results for the main score on the MTEB are presented for all variations of the llm-based embedding. \textbf{The experiment demonstrates that models equipped with Causal Attention and a Multi-Layer Resampler generally outperform others. } However, for specific well-known embedding tasks, models using Bi-directional Attention with a Multi-Layer Resampler show superior performance.}
\label{tab:mteb} 
\end{table*}

==> sections/main_tables/wilcoxon.tex <==

\begin{table*}[h]
\small
\centering
\begin{tabular}{lccccc}
\toprule
Module & STS & Retr. & Clus. & Clas. & Rera. \\
\midrule
\begin{minipage}[t]{6.2cm}Casual Attention + EOS Token Pooling \\ vs.\ Casual Attention + MLR\end{minipage} & 
\begin{minipage}[t]{1.45cm}-0.0118 \\ \textbf{(p=0.0078)}\end{minipage} & 
\begin{minipage}[t]{1.45cm}-0.0135 \\ (p=0.2958)\end{minipage} & 
\begin{minipage}[t]{1.45cm}+0.0244 \\ (p=0.3125)\end{minipage} & 
\begin{minipage}[t]{1.45cm}+0.0033 \\ (p=0.6377)\end{minipage} & 
\begin{minipage}[t]{1.45cm}-0.0050 \\ (p=0.1250)\end{minipage} \\
\addlinespace

\begin{minipage}[t]{6.2cm}Casual Attention + EOS Token Pooling \\ vs.\ Casual Attention + MLR - Layer Weights\end{minipage} & 
\begin{minipage}[t]{1.45cm}-0.0129 \\ \textbf{(p=0.0078)}\end{minipage} & 
\begin{minipage}[t]{1.45cm}-0.0102 \\ (p=1.0000)\end{minipage} & 
\begin{minipage}[t]{1.45cm}+0.0077 \\ (\textbf{p=0.0078})\end{minipage} & 
\begin{minipage}[t]{1.45cm}+0.0035 \\ (p=0.8311)\end{minipage} & 
\begin{minipage}[t]{1.45cm}+0.0017 \\ (p=0.1250)\end{minipage} \\
\addlinespace

\begin{minipage}[t]{6.2cm}Casual Attention + EOS Token Pooling \\ vs.\ Bi-direction Attention + MLR - Layer Weights\end{minipage} & 
\begin{minipage}[t]{1.45cm}-0.0166 \\ \textbf{(p=0.0078)}\end{minipage} & 
\begin{minipage}[t]{1.45cm}-0.0226 \\ \textbf{(p=0.0245)}\end{minipage} & 
\begin{minipage}[t]{1.45cm}+0.0246 \\ (\textbf{p=0.0098})\end{minipage} & 
\begin{minipage}[t]{1.45cm}+0.0143 \\ (p=0.6875)\end{minipage} & 
\begin{minipage}[t]{1.45cm}-0.0075 \\ (p=0.2500)\end{minipage} \\
\addlinespace


\begin{minipage}[t]{6.2cm}Casual Attention + MLR (EOS token) \\ \quad vs.\ Casual Attention + MLR (Last token) \end{minipage} & 
\begin{minipage}[t]{1.45cm}+0.0014 \\ (p=0.6406)\end{minipage} & 
\begin{minipage}[t]{1.45cm}+0.0017 \\ (p=0.5830)\end{minipage} & 
\begin{minipage}[t]{1.45cm}+0.0203 \\ (p=0.5830)\end{minipage} & 
\begin{minipage}[t]{1.45cm}-0.0025 \\ (\textbf{p=0.0010})\end{minipage} & 
\begin{minipage}[t]{1.45cm}-0.0043 \\ (p=0.8750)\end{minipage} \\
\addlinespace

\begin{minipage}[t]{6.2cm}Casual Attention + MLR \\ \quad vs.\ Casual Attention + MLR - Layer Weights \end{minipage} & 
\begin{minipage}[t]{1.45cm}-0.0011 \\ (p=0.3125)\end{minipage} & 
\begin{minipage}[t]{1.45cm}+0.0033 \\ (p=0.6875)\end{minipage} & 
\begin{minipage}[t]{1.45cm}+0.0060 \\ (p=0.8077)\end{minipage} & 
\begin{minipage}[t]{1.45cm}+0.0001 \\ (p=0.0830)\end{minipage} & 
\begin{minipage}[t]{1.45cm}+0.0067 \\ (p=0.1250)\end{minipage} \\

\addlinespace

\begin{minipage}[t]{6.2cm}Casual Attention + MLR\\ \quad vs.\ Bi-direction Attention + MLR \end{minipage} & 
\begin{minipage}[t]{1.45cm}-0.0048 \\ (p=0.1484)\end{minipage} & 
\begin{minipage}[t]{1.45cm}-0.0091 \\ (p=0.6875)\end{minipage} & 
\begin{minipage}[t]{1.45cm}+0.0229 \\ (\textbf{p=0.0166})\end{minipage} & 
\begin{minipage}[t]{1.45cm}+0.0110 \\ (\textbf{p=0.0010})\end{minipage} & 
\begin{minipage}[t]{1.45cm}-0.0025 \\ (p=0.6250)\end{minipage} \\

\addlinespace

\begin{minipage}[t]{6.2cm}Bi-direction Attention + MLR \\ \quad vs.\ Bi-direction Attention + MLR - Layer Weights \end{minipage} & 
\begin{minipage}[t]{1.45cm}+0.8397 \\ (\textbf{p=0.0156})\end{minipage} & 
\begin{minipage}[t]{1.45cm}+0.5607 \\ (p=0.0625)\end{minipage} & 
\begin{minipage}[t]{1.45cm}+0.4010 \\ (p=1.0000)\end{minipage} & 
\begin{minipage}[t]{1.45cm}+0.6761 \\ (\textbf{p=0.0010} \end{minipage} & 
\begin{minipage}[t]{1.45cm}+0.5829 \\ (p=0.6250)\end{minipage} \\


\addlinespace

\begin{minipage}[t]{6.2cm}Casual Attention + MLR - Layer Weights\\ \quad vs.\ Bi-direction Attention + MLR - Layer Weights \end{minipage} & 
\begin{minipage}[t]{1.45cm}+0.0034 \\ (p=0.1484)\end{minipage} & 
\begin{minipage}[t]{1.45cm}-0.0111 \\ (p=0.1563)\end{minipage} & 
\begin{minipage}[t]{1.45cm}+0.0416 \\ (\textbf{p=0.0295})\end{minipage} & 
\begin{minipage}[t]{1.45cm}+0.0448 \\ (\textbf{p=0.0010})\end{minipage} & 
\begin{minipage}[t]{1.45cm}-0.0109 \\ (p=0.3750)\end{minipage} \\

\bottomrule
\end{tabular}
\caption{Wilcoxon Signed Rank Test Results. \newmethod is illustrated with MLR. The score in \textbf{bold} is the significant result. }
\label{tab:wilcoxon}

\end{table*}

